CAFQA: A classical simulation bootstrap for variational quantum algorithms

This work tackles the problem of finding a good ansatz initialization for Variational Quantum Algorithms (VQAs), by proposing CAFQA, a Clifford Ansatz For Quantum Accuracy. The CAFQA ansatz is a hardware-efficient circuit built with only Clifford gates. In this ansatz, the parameters for the tunable gates are chosen by searching efficiently through the Clifford parameter space via classical simulation. The resulting initial states always equal or outperform traditional classical initialization (e.g., Hartree-Fock), and enable high-accuracy VQA estimations. CAFQA is well-suited to classical computation because: a) Clifford-only quantum circuits can be exactly simulated classically in polynomial time, and b) the discrete Clifford space is searched efficiently via Bayesian Optimization. For the Variational Quantum Eigensolver (VQE) task of molecular ground state energy estimation (up to 18 qubits), CAFQA's Clifford Ansatz achieves a mean accuracy of nearly 99% and recovers as much as 99.99% of the molecular correlation energy that is lost in Hartree-Fock initialization. CAFQA achieves mean accuracy improvements of 6.4x and 56.8x, over the state-of-the-art, on different metrics. The scalability of the approach allows for preliminary ground state energy estimation of the challenging chromium dimer (Cr$_2$) molecule. With CAFQA's high-accuracy initialization, the convergence of VQAs is shown to accelerate by 2.5x, even for small molecules. Furthermore, preliminary exploration of allowing a limited number of non-Clifford (T) gates in the CAFQA framework, shows that as much as 99.9% of the correlation energy can be recovered at bond lengths for which Clifford-only CAFQA accuracy is relatively limited, while remaining classically simulable.

==> 2_back.tex <==
\iffalse

\label{appendix}
Section \ref{NTQC} introduces quantum computing basics and errors on today's NISQ devices.
Section \ref{VQA} discusses variational quantum algorithms and their potential suitability to the NISQ era.
Section \ref{Real-VQA} points out that despite VQA suitability to NISQ, they are far from real world usability, especially for VQE molecular chemistry applications. 
Section \ref{bm_ansatz} presents different ansatz choices for VQAs and their benefits and limitations, while Section \ref{bm_bp} focuses on variationally tuning the ansatz and resulting challenges.
Section \ref{bm_init} then discusses how some of the above challenges can be alleviated via effective initialization, as well as limitations of state-of-the-art approaches.
Section \ref{bm_cliff} puts forth ideas of classical simulation for quantum computing and the limited quantum space suited to scalable classical simulation - key to the CAFQA proposal.
Further, Section \ref{bm_ds} discusses search algorithms potentially suited to navigate this classically simulable quantum space.
Finally, Section \ref{ESP} points out specific constraints that molecular chemistry quantum problems might need to satisfy for real usecases. 

\subsection{Near-term Quantum Computing}
\label{NTQC}

The basic unit of quantum information is the quantum bit, or qubit, which can exist in a linear superposition of the basis states $\ket{0}$ and $\ket{1}$. If measured, however, the state $\ket{\psi} = \alpha\ket{0} + \beta\ket{1}$ collapses into either $\ket{0}$ or $\ket{1}$, effectively becoming a classical bit. A system of $n$ qubits requires $2^n$ amplitudes to describe the state. 
Qubits are manipulated via gates which modify the amplitudes. Unlike in classical computation, there are many non-trivial single-qubit gates such as $R_x(\theta)$ and $R_z(\theta)$ which rotate the state around the $x$ and $z$ axes, respectively. Pairs of qubits can be manipulated via multiqubit interactions. The most common of these gates is the two-qubit controlled-$X$, or $CX$. Together with single qubit gates, $CX$ enables universal quantum computation. There are many choices of basis gate sets specified by the underlying hardware \cite{pulse-gokhale2020optimized}. 




% Quantum information science (QIS) redefines the computational model through the use of quantum bits, or qubits, that have two basis states represented as  $\Ket{0} =  \begin{bmatrix}  1 & 0
% \end{bmatrix}^\text{T}$ and $\Ket{1} =  \begin{bmatrix}  0 & 1
% \end{bmatrix}^\text{T}$. Qubits, unlike classical bits that hold a static value of either 0 or 1, demonstrate states of superposition in the form of $\alpha\ket{0} + \beta\ket{1}$ with probability amplitudes $\alpha,\beta \in \mathbb{C}$ and hold values such that $|\alpha|^2+|\beta|^2=1$. Superposition enables $n$ qubits to represent up to $2^n$ states simultaneously, and this phenomenon, along with the ability for quantum states to interfere and become entangled, allow certain problems to be solved with significant reductions in complexity. Qubits hold large quantities of information for processing while in superposition, but upon measurement, quantum state collapses and only classical values of either 0 or 1 are observed.  

% Quantum computation is implemented with operators that cause the probability amplitudes associated with quantum state to evolve. These operators are represented with unitary transformation matrices of size $2^n \times 2^n$ where $n$ is the number of qubits that the operation transforms. 
% Some common single-qubit transformations include the $R_x(\pi)=X$, $R_z(\pi)=Z$, $R_y(\pi)=Y$ rotation operations that cause a bit flip, a phase flip, and a combination bit flip and phase flip, respectively. Additionally, the $H$ gate puts a qubit originally in a basis state into perfect superposition~\cite{mike_ike_2020}. Multi-qubit operations include the logical $SWAP$ operation that causes the exchange of quantum state along with controlled gates, such as $CX$ or $CZ$ that execute an operation on a target qubit depending on the state of one (or more) control  qubit(s).
% If a quantum algorithm were to be thought of as logic circuit composed of gates, the set of gates used for the circuit would depend on the abstraction level used in the description. For example, higher-level circuits that are technology independent may use complex, multi-qubit operators whereas lower-level circuits targeted for execution on quantum hardware will implement a set of elementary single- and two-qubit gates. The set of basis gates used for a particular quantum computer is technology dependent, but it usually consists of a set of single-qubit operations that are capable of implementing arbitrary rotations, $R_x$, $R_y$, and $R_z$, within a small margin of error. The basis set also includes a two-qubit operation such as $CX$ or $CZ$. All quantum computations are possible with a set of basis operations as long as they form a universal gate set.



Current QCs, sometimes called Noisy Intermediate Scale Quantum (NISQ) devices, are error prone and at most around 100 qubits in size~\cite{preskill2018quantum}. These devices are extremely sensitive to external influences and require precise control, and as a result, some of the biggest challenges that limit scalability include limited coherence, gate errors, readout errors, and connectivity. %Systematic error is restrictive, but once the error identified it can be effectively mitigated or corrected in software. The two primary causes of loss of performance are decoherence and crosstalk. 
%Environmental coupling is the source of many errors in quantum systems. For example, amplitude damping describes the sporadic loss of energy resulting in the $\ket{1}$ state falling to the $\ket{0}$ state; the rate of this process is described by the device's $T_1$ time. Similarly dephasing details the sporadic change in relative phase between basis states and is expressed by the $T_2$ time of the device. Both are the cause of decoherence. Finally, crosstalk refers to error caused by simultaneous execution of gates on nearby qubits. The severity of each type of noise varies per qubit and calibration cycle.

With the limited number of qubits available in near-term quantum computers, full-fledged quantum error correction is impractical. 
QEC techniques require uniting multiple physical qubits on a device to act as a single logical qubit and special codes to remedy errors are implemented on these multiple physical qubits.  
Thus the NISQ-era leans towards alternative approaches - specifically error mitigation instead of correction.
%Because of the prototype nature of NISQ devices, we are forced to implement one-to-one mapping for logical and physical qubits.
%As a result, multiple error mitigation techniques have been explored on NISQ devices.
These techniques reduce the effect of noise on the execution of a quantum circuit on the device. 
Unfortunately, the accuracy obtained on NISQ machines, even with the addition of sophisticated error mitigation techniques, is often considerably far from real-world application accuracy requirements, especially when scaled to larger problem sizes with more qubits and deeper circuits~\cite{wang2021error,wang2020noise, kandala2017hardware, ravi2021vaqem}. 





\begin{figure}[!t]
\centering
\fbox{
\includegraphics[width=0.9\columnwidth,trim={0cm 0cm 0cm 0cm}]{figures/VQA.pdf}
}
\caption{Overview of VQA flow that includes quantum and classical processing to minimize some objective function $\braket{H}$, the expectation value of the problem Hamiltonian.}
\label{fig:vqa}
\end{figure}


\subsection{VQA Applications}
\label{VQA}



Variational quantum algorithms are especially important in the near-term because they comply with the constraints of NISQ hardware.
In particular, variational algorithms have innate error resilience, due to the hybrid alternation with a noise-robust classical optimizer~\cite{peruzzo2014variational, mcclean2016theory}. 
A schematic of this process is illustrated in Fig.~\ref{fig:vqa}.
There are multiple applications which are part of the VQA domain such as Quantum Approximate Optimization Algorithm (QAOA)~\cite{farhi2014quantum} and Variational Quantum Eigensolver (VQE)~\cite{peruzzo2014variational}.
While CAFQA is suited widely across variationally algorithms, our discussions and evaluations in this paper primarily focus on VQE.
%We briefly discuss some QAOA results in Section \ref{eval_ovl}.

%\subsubsection{Variational Quantum Eigensolver}

The Variational Quantum Eigensolver (VQE)~\cite{peruzzo2014variational}  is used to compute an upper bound of a Hamiltonian's ground state energy.
This is done by finding a circuit parameterization such that the expectation value of the target Hamiltonian is minimized. 
%This expectation value found is an upper bound for the ground state energy.
Ideally the expectation should be indistinguishable from the ground state energy to the level of accuracy desired~\cite{tilly2021variational}.

This is generally the first step in computing the energy properties of molecules and materials.
The study of electronic structures is critical for quantum chemistry and VQE is therefore relevant for drug discovery, material science, chemical engineering, or nuclear physics.
While conventional computational chemistry provides efficient methods to approximate such properties, they can lack sufficient accuracy in molecular systems due to an inadequate treatment of the correlations between constituent electrons. 
These interactions require computation that scales exponentially in the size of the system, rendering exact quantum chemistry methods generally intractable with conventional computing~\cite{tilly2021variational,PhysRevX.10.041038}.


Thus, VQE is used to find the lowest eigenvalue of a given problem matrix by computing a difficult cost function on the quantum machine and feeding this value into an optimization routine running on a CPU. 
At a high level, VQE can be conceptualized as a guess-check-repeat algorithm \cite{gokhale2019minimizing}. 
The check stage involves the preparation of a quantum state corresponding to the guess.
%where the initial guess is often referred to as the ansatz. 
This preparation stage is done in polynomial time on a quantum computer, but would incur exponential cost  in general on a classical computer. 
This contrast gives rise to a potential quantum speedup for VQE~\cite{Gokhale:2019}.

In this work, we use VQE to primarily target problems from molecular chemistry but also use it to showcase the benefits of CAFQA for optimization tasks like MaxCut. 
The Clifford Ansatz can also be adapted specifically to QAOA\cite{farhi2014quantum} which is better suited to such optimization problems but is not currently pursued.
QAOA uses an ansatz with fixed Clifford gates and its tunable gates can be constrained to be Clifford - thus inherently suited to this work.





\subsubsection{Quantum Approximate Optimization Algorithm}

QAOA~\cite{farhi2014quantum} is an algorithm for generating approximate solutions to optimization problems that are hard to solve exactly.
At an intuitive level, QAOA can be understood as an alternating pattern of mixing and cost-optimization steps. 
At each mixing step, QAOA applies diffusion so that every possible state is explored in quantum superposition. 
At each cost-optimization step, a bias is applied to boost the magnitudes of quantum states that minimize the cost function. 
Thereafter, measuring can yield an approximate solution close to optimal with high probability. 
The number of alternating mixing and cost-optimization rounds is known as $p$. 
%Even for small p, QAOA has competitive results against classical approximation algorithms. 
%For example, at p = 1, QAOA applied to the NP-hard MAXCUT problem yields a cut of size at least 69\% of the optimal cut size. 
%At p = 5, simulations have demonstrated that QAOA achieves mean parity with the best-known classical algorithm, Goemans-Williamson, for 10 node graphs [9]. 
%For larger p, QAOA is expected to outperform classical approximation algorithms even for worst-case bounds, although theoretical guarantees have not been established yet. 
Similar to VQE, QAOA is a guess-check-repeat algorithm. 
%In the case of QAOA, the guesses correspond to the mixing magnitude during iterations 1-$p$ and the cost-optimization magnitude during iterations 1-$p$. 
Each ith mixing iteration is characterized by $\beta$ mixing parameters while each $i$th cost-optimization step is characterized by $\gamma$ cost parameters.
Generally, the performance of the algorithm improves with higher $p$.



\subsection{Real-world accuracy targets for VQE vs NISQ}
\label{Real-VQA}
If a circuit ideally intends to simulate the evolution of some Hamiltonian, $\mathcal{H}$, then in a noisy environment it can be represented as as the evolution of some other Hamiltonian, $\mathcal{H'}$. If noise levels are reasonable and/or if the effects of noise are adequately mitigated, the eigenstates / eigenvalues of $\mathcal{H}$ and $\mathcal{H'}$ will be close in distance.


However, estimating the VQE global optimal with high accuracy has proven challenging in the NISQ era even with sophisticated optimizers, a well-chosen ansatz, and error mitigation. %Cite Kandala? VAQEM? some other papers too...
For instance, the presence of noise considerably worsens the barren plateau problem, impeding fast and accurate convergence~\cite{wang2020noise}. %Coles paper
As an example, ground state energy estimation of molecules (a key use case for VQE) requires energy estimates with an estimation error of less than $1.6 \times 10^{-3}$ Hartree, or what is known as ``chemical accuracy".
Such energy estimates are then used in molecular chemistry for determining properties of chemical reactions and so forth. %\todo{Anything more to add here?}
Unfortunately, the accuracy estimates on NISQ machines are far from accurate, especially as problem size increases. 
For example, prior work on the ground state energy estimation of BeH$_2$ on a superconducting transmon machine results in an error greater than 10$^{-1}$ Hartree, which is roughly 100x lower than the required accuracy~\cite{kandala2017hardware}. %Kandala - plus need more recent work


Although error mitigation methods have shown great success in improving the accuracy of VQE~\cite{ravi2021vaqem,czarnik2020error,Rosenberg2021,barron2020measurement,botelho2021error}, the resulting accuracy is still insufficient for real-world usecases. 
Furthermore, it can significantly increase the resource requirements of the optimization process and can affect its trainability~\cite{wang2021error}. 
It is unclear whether this increase in resources is an acceptable cost or likely to be a critical limitation in larger-scale applications of  VQE~\cite{tilly2021variational,takagi2021fundamental}. %Review / 76


Considering the significant disparity in NISQ-device VQA accuracy and real world requirements, it is imperative to aid VQA methods to the best extent possible.
CAFQA looks to classical simulation for this support and put it to use efficiently in an accurate and scalable manner.










\subsection{Ansatz Parameterized Circuit}
\label{bm_ansatz}

The VQA problem is translated into a task that can be executed on a quantum computer by defining an ansatz wave function that can be implemented on a quantum device as a series of quantum gates - a circuit with parameterized unitary operations is used~\cite{tilly2021variational}. %Review
An ansatz with its parameterized gate rotation angles is shown in Fig.~\ref{fig:ansatz}.
On the one hand, a good ansatz must be sufficiently expressive to appropriately approximate the ground state wave function.
On the other hand, it must not be so expressive that it renders the search for the target state intractable~\cite{tilly2021variational}. 
Further, the ansatz should be suitable in terms of scaling and complexity to today's quantum devices - noise resilience is particularly important in the NISQ era.

In the context of VQE for molecular chemistry, while many ansatz choices are possible, Unitary Coupled Cluster Single-Double (UCCSD), an ansatz motivated by principles of quantum chemistry, is considered the gold standard~\cite{romero2018strategies, Gokhale:2019}. 
Unfortunately the UCCSD ansatz is generally of considerable circuit depth, making it less suitable for today's NISQ machines except for very small molecules like  H$_2$.


More suitable to the NISQ-era are hardware-efficient ansatz like the SU2~\cite{IBM-SU2} which are low depth parameterized circuits that are further hyper-parameterized by the number of qubits, number of repetitions, and type of entanglement, and these can be selected so as to optimize for the quantum application as well as the machine.
While several flavors have been proposed, they follow the fundamentals: the ansatz is constructed by repeating blocks of parameterized single qubit rotation gates, and ladders of entangling gates~\cite{tilly2021variational}.
Hardware efficient ansatz has been used on real NISQ machines targeting molecular chemistry tasks for molecules such as BeH$_2$ with promising ground state energy estimates but not within chemical accuracy~\cite{kandala2017hardware}. %Kandala
The limitation of a hardware efficient anstaz is primarily that it be quite inefficient in its Hilbert space coverage, often requiring a large number of tuning parameters and being limited by barren plateaus~\cite{tilly2021variational, holmes2021connecting}. %[101] 

While many other ansatz structures are possible, CAFQA builds atop a traditional hardware efficient ansatz~\cite{kandala2017hardware}.
Suitability to other ansatz structures is discussed in Section \ref{FW}.







\subsection{Parameter Space, Classical Tuning and Barren Plateaus}
\label{bm_bp}
The execution on the quantum processor evaluates the VQA objective function to be optimized classically.
The parameter space for classical optimization is determined by the ansatz.
The space is continuous and grows exponentially in the number of qubits.
%Further, even if surfaces are smooth in the ideal case, noise can change this landscape considerably.
For simple VQA problems and in the presence of minimal noise, the optimization surface is convex around the global minimum and smooth~\cite{9259985}. 
As noise increases, in line with NISQ machines, the optimization surface can potentially become non-convex and non-smooth. 
The surface contour worsens as the problem complexity increases because of increase in circuit depth, number of parameters (and thus the likelihood of noise-induced local minima), and entanglement spread out over many qubits (causing noise effects to become non-local)~\cite{9259985}.

A good optimizer has a short distance to the true global optimum and high accuracy of the optimal parameters found.
A variety of classical optimizers which perform fairly well on NISQ machines are discussed in ~\cite{9259985}.
Even with good optimizers, VQAs often suffer from a barren plateau problem. 
The barren plateau is the phenomenon that the gradients of the VQE parameters vanish exponentially.
This could occur in increasing fashion with the number of qubits~\cite{mcclean2018}, in the expressibility of the ansatz~\cite{Holmes2016}, the degree of entanglement of the wavefunction~\cite{PhysRevResearch.3.033090,marrero2021entanglement}, or non-locality of the cost function~\cite{Cerezo2021,Uvarov2021}. 
Important to this work, barren plateaus can become an especially significant problem in the presence of noise~\cite{wang2020noise} and with poor (random) ansatz initialization~\cite{mcclean2018}.
%More details about the above are discussed in Section \ref{RW}.
Thus, well-chosen initialization of the ansatz can help avoid barren plateaus, apart from other effects of noise, and therefore enable faster and more accurate convergence on the VQA problem.






\subsection{Ansatz Initialization}
\label{bm_init}
Once a parameterized circuit is selected, the circuit parameters have to be initialized in a suitable manner.
As discussed above, a poor choice of parameters can lead to barren plateaus and slow / suboptimal convergence.
A popular and simple approach to construct the initial state for quantum systems is from Hartree-Fock (HF) theory~\cite{hartree1935self}.
HF yields a single Slater-determinant approximation to the ground state of a quantum system.
While such approximation / optimization problems are generically hard, HF usually rapidly converges to a near-optimal solution, especially for closed-shell molecules at equilibrium geometries~\cite{Microsoft-HF}.
HF yields a quantum state that has no entanglement between the electrons - HF assumes that each electron’s motion can be described by a single-particle function (orbital), independent of the instantaneous motion of other electrons.
By assuming a single-determinant form for the wavefunction, HF neglects correlation between electrons, which is where classical computing is limited in solving such molecular chemistry problems.
%The electrons are in fact subject to an average non-local potential arising from the other electrons, which can lead to a poor description of the electronic structure. 
Thus, although HF is qualitatively correct in many materials and compounds, it is generally insufficient to make accurate quantitative predictions~\cite{Ornl-HF}. %https://web.ornl.gov/~kentpr/thesis/pkthnode13.html
Therefore, obtaining accurate results, especially for strongly correlated systems and/or away from equilibrium geometry, necessitate quantum states that go beyond HF.
CAFQA is one novel approach to do so, achieving both qualitative and quantitative accuracy.
%https://docs.microsoft.com/en-us/azure/quantum/user-guide/libraries/chemistry/concepts/hartree-fock




        %\todo{Would be nice to have a table here showing best estimates on NISQ machines}

\subsection{Classical Simulation and the Clifford Space}
\label{bm_cliff}

Classical simulators are important to the quantum computing stack. 
Methods include simulating partial or entire state vector evolution during computation, as well as full unitary simulation with or without noise. 
Simulations are then used to verify quantum computations, model noise, develop and test quantum algorithms, and so on~\cite{alexeev2021quantum}. %https://journals.aps.org/prxquantum/pdf/10.1103/PRXQuantum.2.017001
Classical simulation usually requires exponential resources (otherwise the need for a quantum computer is obviated) and thus are only useful for simulating small quantum systems.
Even using high-performance supercomputers, simulation is restricted to under 100 qubits~\cite{tilly2021variational,Haner2017,Raedt2019,Boixo2018,45919}.
%More details on these can be found in Section \ref{}.

However, not all simulation is non-scalable. 
The Gottesman-Knill’s theorem states that, \emph{``Any quantum computer performing only: a) Clifford group gates, b) measurements of Pauli group operators, and c) Clifford group operations conditioned on classical bits, which may be the results of earlier measurements, can be perfectly simulated in polynomial time on a probabilistic classical computer"}~\cite{gottesman1998heisenberg}. %https://arxiv.org/pdf/quant-ph/9807006v1.pdf 

While the Clifford group operations and Pauli group measurements do not provide a universal set of quantum gates there are quantum domains that have applications focused on the Clifford-space including quantum communications / networks~\cite{Veitch2014}, error correction codes~\cite{QECIntro}, teleportation~\cite{gottesman1999demonstrating} and error mitigation~\cite{czarnik2020error,strikis2021learningbased}.

CAFQA explores the benefits of Clifford-only circuits as an ansatz for variational algorithms.
While it is a limited discrete tuning space, we observe such an ansatz to be tremendously effective in approaching required accuracy over a variety of applications.
While we have restricted the ansatz to strictly the Clifford group in this paper, there is potential to introduce a small number of non-Clifford gates as well~\cite{Bravyi2016}. %Two papers from related work.
Such an ansatz could provide even greater accuracy before actual execution on the (noisy) quantum device.
More details in Section \ref{FW}.

\subsection{Search Algorithms}
\label{bm_ds}

To efficiently search through the discrete Clifford parameter space, CAFQA requires a sample-efficient search technique to find the performant ansatz parameters as quickly as possible. 
Bayesian optimization is such a technique that actively and intelligently queries the most informative samples at each round to reduce the number of samples required~\cite{frazier2018tutorial}. 
Due to this merit, Bayesian optimization has been successfully applied to different domains in computer systems optimization such as compiler tuning~\cite{nardi2019practical}, resource allocation~\cite{Clite2020}, and configuration optimization~\cite{dingbayesian,ding2021,cherrypick2017,Bliss2021}.
% make use of a sample-efficient, black-box, gradient-free search algorithm suited to discrete search.
%Thus searching through the Clifford space for optimal tuning parameters requires efficient discrete search algorithms.
% Potential techniques include genetic algorithms~\cite{ga}, simulated annealing~\cite{sa} and Bayesian Optimization methods~\cite{nardi2019practical, dingbayesian,BO-1,BO-2,BO-3}.
%Some of these techniques as well as some prior quantum computing usecases are discussed  in Section \ref{RW}.
Bayesian optimization iteratively alternates between intelligent sampling and model updates. 
As such, it includes two components: a surrogate model and an acquisition function. 
The surrogate model tries to learn the unknown underlying function that maps the search parameters to the problem objective.
Popular surrogate models include random forests and Gaussian processes.
Random forests are inherently suited to a discrete search space and are the surrogate of choice in this work.
The acquisition function is the search strategy that selects the next sample to query to update the surrogate model. 
% A suitable acquisition function is chosen based on the appropriate exploration and exploitation trade-off for a given problem.
CAFQA uses a greedy acquisition function~\cite{nardi2019practical,ding2021}.
CAFQA specific details of the BO search are discussed in Section \ref{DS-proposal}.

% We search the Clifford space efficiently via Bayesian Optimization (BO) using a Random Forest surrogate model and a greedy acquisition function.
% BO is a form of semi-supervised machine learning which alternatively uses a small number of training examples to achieve high prediction accuracy.
% A surrogate function is an approximation of the unknown contour of the problem objective and is modeled via the iterative training.
% BO requires a surrogate model that is flexible and accurate to model complex interactions of different types of configuration parameters.
% In this work we choose a Random forest surrogate.
% Random forests are made up of decision trees which learn to regress data points based on a set of training examples. 
% Combining many weak regressors creates a forest which allows approximating highly non-linear functions with high accuracy. 
% Random forests naturally deal with categorical and discrete variables which are important in computer systems optimization~\cite{nardi2019practical} and useful to the discrete search in this work.
% The surrogate function is updated with an acquisition function which identifies new training samples to test in a trade-off of exploration and exploitation. 
% This work uses a greedy approach~\cite{nardi2019practical,ding2021} which provides a good trade-off between the above.


%We note that there is potential to improve upon our chosen search technique to enable better scaling to larger problem sizes, as discussed in Section \ref{FW}, but is beyond our current scope. \yd{do we need this sentence?}


\subsection{Electron and Spin Preservation Constraints}
\label{ESP}


For a given molecular system, the Fock space combines the Hilbert spaces of molecular forms with all possible numbers of electrons and all electron spin combinations.
The Hamiltonian of a molecule M has eigenvalues which correspond to the electronic energies of different molecular states such as M, M$^{+}$, M$^{-}$ and so on~\cite{ryabinkin2018constrained}.
When given the molecular Hamiltonian as above and solving VQE for the upper bond of the ground state energy of simple neutral molecules, the lack of specific electron preservation constraints does not prove to be detrimental because the energy of the neutral molecule is usually lower than that of corresponding cations (otherwise the molecule would auto-ionize) and is also often lower than that of corresponding anions (unless the molecule has high positive electron affinity).
On the other hand, when solving for energy estimates of cations and anions explicit enforcement of electron preservation constraints is often required.
Similarly, with respect to electron spin, the spin multiplicity of the lowest energy state could be different from specific target multiplicities.
Thus, it is important to consider constraining the number of electrons and/or their spins if required for the problem at hand. 
CAFQA ensures that that any required constraints are maintained, along the lines of prior work~\cite{ryabinkin2018constrained}.

For Hartree Fock, we note that the HF solution is the lowest single determinant energy solution for the specified number of electrons. 
The general HF solution should produce the computational basis with the lowest energy solution irrespective of spin, whereas specific implementations might constrain spin multiplicities as well.

To our knowledge, the above preservation constraints / differentiations are sometimes ignored in prior work - leading to comparisons between proposed solutions with no spin and electron constraints against a HF method with specific constrains, thereby potentially showing magnified benefits.
We specifically differentiate among these scenarios in our evaluations.
\fi

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

